RichWasm: Bringing Safe, Fine-Grained, Shared-Memory Interoperability Down to WebAssembly

Safe, shared-memory interoperability between languages with different type systems and memory-safety guarantees is an intricate problem as crossing language boundaries may result in memory-safety violations. In this paper, we present RichWasm, a novel richly typed intermediate language designed to serve as a compilation target for typed high-level languages with different memory-safety guarantees. RichWasm is based on WebAssembly and enables safe shared-memory interoperability by incorporating a variety of type features that support fine-grained memory ownership and sharing. RichWasm is rich enough to serve as a typed compilation target for both typed garbage-collected languages and languages with an ownership-based type system and manually managed memory. We demonstrate this by providing compilers from core ML and L3, a type-safe language with strong updates, to RichWasm. RichWasm is compiled to regular Wasm, allowing for use in existing environments. We formalize RichWasm in Coq and prove type safety.

==> exec2.tex <==
{\scriptsize
\[\begin{array}{r l l}
%variants
 \redrule{v~\Wvariantmalloc{j}{\many{\Wty}}{q}}{\Wmalloc{(32 + \sz{v})}{\WHVvariant{j}{v}}{q}} \\
% variant case unr
\redrule
{
\WVref{l_{\Wunr}}~\manyn{v}{n}~\Wvariantcase{\Wunr}{\WHvariant{\manyn{\Wtau}{m}}}{\Warrow{\manyn{\Wtau_1}{n}}{\many{\Wtau_2}}}{\Wleff}
{\manyn{(\many{e})}{m}}}
{\WVref{l_{\Wunr}}~\manyn{v}{n}~\Wblock{\Warrow{\manyn{\Wtau_1}{n}}{\many{\Wtau_2}}}{\Wleff}{v'~\manyn{(\many{e})}{m}_{.i}}} \\
 & & \hfill \text{where } {(s_{\Wkey{mem}})_{\Wunr}(l)  = \WHVvariant{i}{v'}} \\
% variant case lin
 \redrule{
  \WVref{l_{\Wunr}}~\manyn{v}{n}~\Wvariantcase{\Wlin}{\WHvariant{\manyn{\Wtau}{m}}}{\Warrow{\manyn{\Wtau_1}{n}}{\many{\Wtau_2}}}{\Wleff}
  {\manyn{(\many{e})}{m}}
  }
  {\WVref{l_{\Wlin}}~\Wfree~\manyn{v}{n}~\Wblock{\Warrow{\manyn{\Wtau_1}{n}}{\many{\Wtau_2}}}{\Wleff}{v'~\manyn{(\many{e})}{m}_{.i}}}  \\
 & & \hfill{\text{where }  (s_{\Wkey{mem}})_{\Wlin}(l)  = \WHVvariant{i}{v'}} \\
 & & \hfill {s' = s \text{ with } \Wkey{mem}_{\Wlin}(l) = \WHVarray{0}{\epsilon}} \\
% arrays 
 \redrule{v~\Wkey{ui32.const}~n~\Warraymalloc{q}}{\Wmalloc{(j\times\sz{v})}{\WHVarray{j}{\manyn{v}{j}}}{q}} \\
% array get
 \redrule{(\WVref{l_{mem}})~(np.\Wkey{const}\ j)~\Warrayget}
{(\WVref{l_{mem}})~v_j} \\
 & & \hfill  \text{where }{\WHVarray{i}{(v_0 \dots v_j \dots)} = (s_{\Wkey{mem}})_{mem}(l)} \\
% array get trap
 \redrule{(\WVref{l_{mem}})~(np.\Wkey{const}\ j)~\Warrayget}
{\Wtrap} \\
 & & \hfill \text{where }  {\WHVarray{i}{\many{v}} = (s_{\Wkey{mem}})_{mem}(l)} \\
 & & {j\geq i\text{ or }j < 0} \\
% array set
 \redrule{s;\many{v};\many{sz};(\WVref{l_{mem}})~(np.\Wkey{const}\ j)~v~\Warrayset}
{s';\many{v};\WVref{l_{mem}}} \\
 & & \hfill \text{where } {\WHVarray{i}{v_0\dots v_{j-1} v_j\dots} = (s_{\Wkey{mem}})_{mem}(l)} \\
 & & \hfill {s' = s \text{ with } \Wkey{mem}_{mem}(l) = \WHVarray{i}{v_0\dots v_{j-1} v\dots}} \\
% array set trap
 \redrule{(\WVref{l_{mem}})~(np.\Wkey{const}\ j)~\Warrayset}
{\Wtrap} \\
 & & \hfill \text{where }  {\WHVarray{i}{\many{v}} = (s_{\Wkey{mem}})_{mem}(l)} \\
 & & \hfill {j\geq i\text{ or }j < 0} \\
% exists 
 \redrule{v~\Wexistpack{\Wpty}{\Whty}{q}}{\Wmalloc{(64+\sz{v})}{\WHVpack{\Wpty}{v}{\Whty}}{q}}\\
% unpack unr
 {s;\many{v};\many{sz};\manyn{v}{n}~(\WVref{l_{\Wunr}})} \\
 \redrule{\Wexistunpack{\Wunr}{\Whty}{tf}{\Wleff}{\Wptyvar}{\many{e}}}
{s;\many{v};(\WVref{l_{\Wunr}})~\manyn{v}{n}~
  \Wblock{tf}{\Wleff}{v'~\sbst{\Wptyvar}{\Wpty}{\many{e}}}} \\
 & & \hfill{\text{where } \WHVpack{\Wpty}{v'}{\Whty} = (s_{\Wkey{mem}})_{\Wunr}(l)} \\
 & & \hfill tf = {\Warrow{\manyn{\Wtau_1}{n}}{\many{\Wtau_2}}} \\
% unpack lin
 {s;\many{v};\many{sz};(\WVref{l_{\Wlin}})} \\
 \redrule{\Wexistunpack{\Wlin}{\Whty}{tf}{\Wleff}{\Wptyvar}{\many{e}}}
{s';\many{v};v'~(\WVref{l_{\Wlin}})~\Wfree~
  \Wblock{tf}{\Wleff}{\sbst{\Wptyvar}{\Wpty}{\many{e}}}} \\
 & & \hfill{\text{where } \WHVpack{\Wpty}{v'}{\Whty} = (s_{\Wkey{mem}})_{\Wlin}(l)} \\
 & & \hfill {s' = s \text{ with } \Wkey{mem}_{\Wlin}(l) = \WHVarray{0}{\epsilon}} \\
 & & \hfill tf = \Warrow{\many{\Wtau_1}}\many{\Wtau_2} \\
 & & \hfill tf' = \Warrow{\manyn{\Wtau_1}{n}~\sbst{\Wptyvar}{\Wpty}{\Wtau_v}}{\many{\Wtau_2}} \\
% qualify
 \redrule{v~\Wqualify{q}}{v} \\
%
% free
 \redrule{s;\many{v};\many{sz};(\WVref{l_{\Wlin}})~\Wfree}{s';\many{v};\epsilon}
\hfill  \text{~where }  \\
 & & \hfill {s' = s \text{ with } l\notin\text{dom}(\Wkey{mem}_{\Wlin})} \\
% malloc
 \redrule{s;\many{v};\many{sz};\Wmalloc{\Wsz}{hv}{mem}}{s';\many{v};\WVmempack{l}{(\WVref{l_{mem}})}} \\
 & & \hfill \text{where } {s' = s \text{ with } \Wkey{mem}_{mem}(l) = hv} \\
% malloc trap
\end{array}\]
}

